Calibrating hypersonic turbulence flow models with the HIFiRE-1 experiment using data-driven machine-learned models

In this paper we study the efficacy of combining machine-learning methods with projection-based model reduction techniques for creating data-driven surrogate models of computationally expensive, high-fidelity physics models. Such surrogate models are essential for many-query applications e.g., engineering design optimization and parameter estimation, where it is necessary to invoke the high-fidelity model sequentially, many times. Surrogate models are usually constructed for individual scalar quantities. However there are scenarios where a spatially varying field needs to be modeled as a function of the model's input parameters. We develop a method to do so, using projections to represent spatial variability while a machine-learned model captures the dependence of the model's response on the inputs. The method is demonstrated on modeling the heat flux and pressure on the surface of the HIFiRE-1 geometry in a Mach 7.16 turbulent flow. The surrogate model is then used to perform Bayesian estimation of freestream conditions and parameters of the SST (Shear Stress Transport) turbulence model embedded in the high-fidelity (Reynolds-Averaged Navier-Stokes) flow simulator, using wind-tunnel data. The paper provides the first-ever Bayesian calibration of a turbulence model for complex hypersonic turbulent flows. We find that the primary issues in estimating the SST model parameters are the limited information content of the heat flux and pressure measurements and the large model-form error encountered in a certain part of the flow.

==> macros.tex <==
%!TEX root = paper.tex

\DeclareMathOperator{\arccosh}{arccosh}
\newcommand{\qtext}[1]{\quad\text{#1}\quad}

% Specific Spaces
\newcommand{\SH}{\mathcal{H}} %Hyperbolic
\newcommand{\SV}{\mathcal{V}} %Vertices
\newcommand{\SL}{\mathcal{L}} %Landmarks
\newcommand{\SN}{\mathcal{N}} %Non-Landmarks
\newcommand{\SA}{\mathcal{A}}
\newcommand{\SB}{\mathcal{B}}
\newcommand{\SJ}{\mathcal{N}}
\newcommand{\SR}{\mathcal{R}}

% Specific Matrices
\newcommand{\MU}{\mathbf{U}}
\newcommand{\MUA}{\mathbf{U}_{\SA}}
\newcommand{\MUV}{\mathbf{U}_{\SV}}
\newcommand{\MUL}{\mathbf{U}_{\SL}}

% Specific Vectors
\newcommand{\Vu}{\mathbf{u}}
\newcommand{\Vv}{\mathbf{v}}
\newcommand{\Vs}{\mathbf{s}}

% Specific error functions
\newcommand{\Eij}{e(\Vu_i,\Vu_j,\kappa)}
\newcommand{\Euv}{e(\Vu,\Vv,\kappa)}
\newcommand{\Evu}{e(\Vv,\Vu,\kappa)}
\newcommand{\EAj}[1][\SA]{\hat E_{#1}(\Vu_j,\kappa)}
\newcommand{\Ej}[1][j]{\hat E_{#1}(\Vu_j,\kappa)}
\newcommand{\EAu}[1][\SA]{\hat E_{#1}(\Vu,\kappa)}
\newcommand{\EAjalt}[1][\SA]{\hat E_{#1}(\Vu_j)}
\newcommand{\EAjtilde}[1][\tilde{\SA}]{\hat E_{#1}(\Vu_j)}
\newcommand{\EA}[1][\SA]{E_{#1}(\MU_{#1},\kappa)}
\newcommand{\EAr}[1][\SA_r]{E_{#1}(\MU_{#1},\kappa)}

% Gradient
\newcommand{\Grad}[2]{\frac{ \partial #1 }{\partial #2}}

% % Theorem and Proof
% \newtheorem{theorem}{Theorem}
% \newenvironment{proof}{\smallskip\par\noindent\emph{Proof.}}{}

\newcommand{\Note}[1]{\textcolor{red}{#1}}

% for comments in algorithm2e environment
\usepackage{algpseudocode}
\algrenewcommand\textproc{\texttt}
\renewcommand{\algorithmiccomment}[1]{\hfill\color{gray}{$\#\;$\textit{#1}}\color{black}}
% \MakeRobust{\Call}
\newcommand{\FunCall}[2]{ \texttt{#1}(#2)}
\algnewcommand{\IFor}[1]{\State\algorithmicfor\ #1}
\algnewcommand{\EndIFor}{\unskip\ \algorithmicend\ \algorithmicfor}


% ----------------------------------------
% TiKZ/PGFPlots Stuff
% ----------------------------------------

\usepackage{xparse}

% --------------------
% Define plot styles for addplot+
% --------------------
% Adapted from http://tex.stackexchange.com/questions/134346/different-marker-shape-for-pgf-tikz
\pgfplotscreateplotcyclelist{my cycle}{%
solid, every mark/.append style={solid,fill=.!25}, mark=*\\%
dotted, every mark/.append style={solid, fill=.!25}, mark=square*\\%
densely dotted, every mark/.append style={solid, fill=.!25}, mark=otimes*\\%
loosely dotted, every mark/.append style={solid, fill=.!25}, mark=triangle*\\%
dashed, every mark/.append style={solid, fill=.!25},mark=diamond*\\%
loosely dashed, every mark/.append style={solid, fill=.!25},mark=*\\%
densely dashed, every mark/.append style={solid, fill=.!25},mark=square*\\%
dashdotted, every mark/.append style={solid, fill=.!25},mark=otimes*\\%
dashdotdotted, every mark/.append style={solid},mark=star\\%
densely dashdotted,every mark/.append style={solid, fill=.!25},mark=diamond*\\%
}

% --------------------
% Special command for adding legend entry that requires macro expansion
% --------------------
\newcommand{\addlegendentrywm}[1]{\edef\temp{\noexpand\addlegendentry{#1}}\temp}

% --------------------
% Graph list to cycle through
% --------------------
\def\graphlist{Amazon,DBLP,LiveJournal,Orkut,Youtube}
\def\graphlistplus{Amazon,DBLP,LiveJournal,Orkut,Youtube,Friendster}
\def\graphlistbig{Friendster}

% --------------------
% Colors
% --------------------
%\definecolor{hypy-color}{HTML}{E41A1C}
%\definecolor{rigel-color}{HTML}{377EB8}

\definecolor{hypy-color}{rgb}{0.2235, 0.4157, 0.6941}
\definecolor{rigel-color}{rgb}{0.8549, 0.4863, 0.1882}
\definecolor{hypy-color-fixed-k}{RGB}{57, 193, 138}

\definecolor{hypy-color-L200}{RGB}{77, 31, 242}
\definecolor{hypy-color-L400}{RGB}{45, 214, 130}
\definecolor{hypy-color-L800}{RGB}{240, 17, 240}
\definecolor{hist-color}{RGB}{0, 128, 0}


% --------------------
% Axis styles, ticks, etc.
% --------------------
\pgfplotsset{every axis/.append style={
    % Adapted from http://tex.stackexchange.com/questions/300669/how-can-i-change-font-size-on-x-y-labels
    legend style={font=\footnotesize},
    label style={font=\footnotesize},
    tick label style={font=\footnotesize},
    title style={font=\footnotesize},
    % Adapted from http://tex.stackexchange.com/questions/142120/positioning-of-pgfplot-axis-labels
    %x label style={at={(axis description cs:0.5,-0.07)},anchor=north},
    %y label style={at={(axis description cs:-0.07,.5)},anchor=south},
}}

\usetikzlibrary{pgfplots.groupplots}

\DeclareDocumentCommand \ValidationHopPlotsHypy { t* m m m m D[]{2.5in}}{%
  \def\graphname{#2}%
  \def\edim{#3}
  \def\rigeledim{#4}%
  \def\gbarwidth{#5}%
  \def\xwidth{#6}
  \subfloat[{\graphname}]{\label{fig:hops-\graphname}%
    \begin{tikzpicture}
      \begin{groupplot}[
        group style = {
          group size = 1 by 2,       
          x descriptions at=edge bottom,
          vertical sep=0.2cm,
        },
        scaled ticks=false,
        width=\xwidth,
        height=2in,     
        % ybar, 
        % /pgf/bar width=\gbarwidth, 
        xlabel=Hops,
        xtick align=inside,
        cycle list name = my cycle,
        ]
        \nextgroupplot[\IfBooleanTF{#1}{}{ylabel=Pair Count (Thousands)}]
        \addplot[draw=hist-color,fill=hist-color,opacity=.5,ybar,/pgf/bar width=\gbarwidth]
        table[x = hops, y expr = \thisrow{vertices_per_hop}/1000]{../figdata/hypy_\graphname_L100_dim\edim_hist_data.txt};
        
        \nextgroupplot[\IfBooleanTF{#1}{}{ylabel=MSE},ymode=log]
        \addplot+[hypy-color,opacity=1]%,mark min=above]
        table[x = hops, y = MSE_per_hop] {../figdata/hypy_\graphname_L100_dim\edim_hist_data.txt}; 
        \addlegendentry{Hypy $d=\edim$}
        \pgfplotsset{cycle list shift=-1}

        \addplot+[rigel-color,opacity=1]%,mark min=above]
        table[x = hops, y = MSE_per_hop] {../figdata/rigel_\graphname_L100_dim\rigeledim_hist_data.txt}; 
        \addlegendentry{Rigel $d=\rigeledim$}

      \end{groupplot}      
    \end{tikzpicture}%
  }%
}

\DeclareDocumentCommand \ValidationHopPlotsHypyL { t* m m m m m D[]{2.5in} m}{%
  \def\graphname{#2}%
  \def\edima{#3}
  \def\edimb{#4}
  \def\edimc{#5}
  \def\gbarwidth{#6}%
  \def\xwidth{#7}
  \def\ymax{#8}%
  \subfloat[{\graphname\@ ($d=\edima, \edimb, \edimc$)}]{\label{fig:hopsL-\graphname}%
    \begin{tikzpicture}
      % \begin{semilogyaxis}
      \begin{groupplot}
          [
          group style = {
            group size = 1 by 2,       
            x descriptions at=edge bottom,
            vertical sep=0.2cm,
          },
          scaled ticks=false,
          width=\xwidth,
          height=2in,     
          % ybar, 
          % /pgf/bar width=\gbarwidth, 
          xlabel=Hops,
          xtick align=inside,
          % ymax = \ymax,
          ymin = 0,
          cycle list name = my cycle,
          ]
          \nextgroupplot[\IfBooleanTF{#1}{}{ylabel=Pair Count (Thousands)}]
          \addplot[draw=hist-color,fill=hist-color,opacity=.5,ybar,/pgf/bar width=\gbarwidth]
          table[x = hops, y expr = \thisrow{vertices_per_hop}/1000] {../figdata/hypy_\graphname_L100_dim\edima_hist_data.txt};
          
          \nextgroupplot[\IfBooleanTF{#1}{}{ylabel=MSE},ymode=log]
          \addplot+[hypy-color,opacity=1,mark min=above]
          table[x = hops, y = MSE_per_hop] {../figdata/hypy_\graphname_L100_dim\edima_hist_data.txt};
          \addlegendentry{$\ell = 100$}

          \addplot+[hypy-color-L400,opacity=.5]%,mark min=above]
          table[x = hops, y = MSE_per_hop] {../figdata/hypy_\graphname_L400_dim\edimb_hist_data.txt}; 
          \addlegendentry{$\ell = 400$}

          \addplot+[hypy-color-L800,opacity=.6]%,mark min=above]
          table[x = hops, y = MSE_per_hop] {../figdata/hypy_\graphname_L800_dim\edimc_hist_data.txt}; 
          \addlegendentry{$\ell = 800$}
      \end{groupplot}      
      % \end{semilogyaxis}
    \end{tikzpicture}%
  }%
}

\DeclareDocumentCommand \MSEPlots { m D[]{2.5}}{%
  \def\graphname{#1}%
  \def\ymax{#2}%
  \subfloat[\graphname]{\label{fig:mse-\graphname}%
    \begin{tikzpicture}
      \begin{groupplot}[group style = {
          group size = 3 by 1,
          y descriptions at=edge left,
          horizontal sep = 0.2cm,
        },
        height=2in, width=2in,
        xtick = {2,4,...,10},
        minor x tick num = {1},
        ylabel = MSE,
        xlabel = Dimension,
        legend pos = north east,
        cycle list name = my cycle,
        ymax = \ymax,
        ymin = 0,
        ]
        \nextgroupplot[title=Landmarks]
        \addplot+[rigel-color,error bars/.cd,y dir = both,y explicit] %
        table[x expr = \thisrow{dimension}+0.15, y = landmark_MSE, y error = landmark_SSE]
        {../figdata/rigel_\graphname_L100_data.txt};
        \pgfplotsset{cycle list shift=-1}
        \addplot+[hypy-color,error bars/.cd,y dir = both,y explicit] %
        table[x expr = \thisrow{dimension}-0.15, y = landmark_MSE, y error = landmark_SSE]
        {../figdata/hypy_\graphname_L100_data.txt};

        \nextgroupplot[title=Nonlandmarks]
        \addplot+[rigel-color,error bars/.cd,y dir = both,y explicit] %
        table[x expr = \thisrow{dimension}+0.15, y = nonlandmark_MSE, y error = nonlandmark_SSE]
        {../figdata/rigel_\graphname_L100_data.txt};
        \pgfplotsset{cycle list shift=-1}
        \addplot+[hypy-color,error bars/.cd,y dir = both,y explicit] %
        table[x expr = \thisrow{dimension}-0.15, y = nonlandmark_MSE, y error = nonlandmark_SSE]
        {../figdata/hypy_\graphname_L100_data.txt};

        \nextgroupplot[title=Validation]
        \addplot+[rigel-color,mark min=above]%,mark options={solid,fill opacity=0}]
        table[x = dimension, y = validation_MSE]
        {../figdata/rigel_\graphname_L100_data.txt};
        
        \addlegendentry{Rigel, $\ell = 100$}
        
        \pgfplotsset{cycle list shift=-1}
        \addplot+[hypy-color,mark min=below]
        table[x = dimension, y = validation_MSE]
        {../figdata/hypy_\graphname_L100_data.txt};
        
        \addlegendentry{Hypy, $\ell = 100$}


      \end{groupplot}      
    \end{tikzpicture}%
  }%
}

\DeclareDocumentCommand \MSEPlotsfixedk { m m}{%
  \def\graphname{#1}%
  \def\ymax{#2}%
  \subfloat[\graphname]{%\label{fig:kappa:\graphname}
  \label{fig:msekixedk-\graphname}%
    \begin{tikzpicture}
      \begin{axis}
        [
        height=2in, width=2in,
        xtick = {2,4,...,10},
        minor x tick num = {1},
        xlabel = Dimension,
        ylabel = MSE,
        legend pos = north east,
        cycle list name = my cycle,
        %ymode=log,
        yminorticks=true,
        %ymax = 10,
        ymax = \ymax,
        ymin = 0,
        ]
        \addplot+[hypy-color,error bars/.cd,y dir = both,y explicit] %
        table[x expr = \thisrow{dimension}-0.15, y = landmark_MSE]
        {../figdata/k_tests/hypy_\graphname_L100_data_var_k.txt};
        \addlegendentry{$\kappa$ varies}

        \pgfplotsset{cycle list shift=-1}
        \addplot+[hypy-color-fixed-k,error bars/.cd,y dir = both,y explicit] %
        table[x expr = \thisrow{dimension}+0.15, y = landmark_MSE]
        {../figdata/k_tests/hypy_\graphname_L100_data_fixed_k.txt};
        
        \addlegendentry{$\kappa=1$}


      \end{axis}    
    \end{tikzpicture}%
}}

\newcommand{\ErrorPlot}[3]{%
  \def\graphname{#1}%
  \def\typename{#2}%
  \def\nlandmarks{#3}%
  \subfloat[#1: #2]{\label{fig:mse-#1-#2}%
    \begin{tikzpicture}
      \begin{axis}[
        height=2in, width=2in,
        xtick = {2,4,...,10},
        minor x tick num = {1},
        xlabel = Embedding Dimension,
        ylabel = MSE,
        legend pos = north east,
        cycle list name = my cycle,
        ]
        %
        \addplot+[rigel-color,error bars/.cd,y dir = both,y explicit] %
        table[x expr = \thisrow{dimension}+0.15, y = \typename_MSE, y error plus = \typename_SSE, 
        y error minus expr = {min(\thisrow{\typename_SSE},\thisrow{\typename_MSE})}]
        {../figdata/rigel_\graphname_L100_data.txt};
        %
        \addlegendentry{Rigel, $\ell = 100$}
        %
        \pgfplotsset{cycle list shift=-1}
        \addplot+[hypy-color,error bars/.cd,y dir = both,y explicit] %
        table[x expr = \thisrow{dimension}-0.15, y = \typename_MSE, y error plus = \typename_SSE, 
        y error minus expr = {min(\thisrow{\typename_SSE},\thisrow{\typename_MSE})}]
        {../figdata/hypy_\graphname_L\nlandmarks_data.txt};
        %
        \addlegendentry{Hypy, $\ell = $\nlandmarks}
        %
      \end{axis}
    \end{tikzpicture}%
  }%
}
\newcommand{\ValidationPlot}[2]{%
  \def\graphname{#1}%
  \def\nlandmarks{#2}%
  \subfloat[#1: validation]{
    \begin{tikzpicture}
      \begin{axis}[
        height=2in,width=2in,
        xtick = {2,4,...,10},
        minor x tick num = {1},
        xlabel = Embedding Dimension,
        ylabel = MSE,
        legend pos = north east,
        cycle list name = my cycle,
        ]
        
        \addplot+[rigel-color,mark min=above]%,mark options={solid,fill opacity=0}]
        table[x = dimension, y = validation_MSE]
        {../figdata/rigel_\graphname_L100_data.txt};
        
        \addlegendentry{Rigel, $\ell = 100$}
        
        \pgfplotsset{cycle list shift=-1}
        \addplot+[hypy-color,mark min=below]
        table[x = dimension, y = validation_MSE]
        {../figdata/hypy_\graphname_L\nlandmarks_data.txt};
        
        \addlegendentry{Hypy, $\ell = $\nlandmarks}
        
      \end{axis}
    \end{tikzpicture}
  }%
}
\newcommand{\ValidationPlotCompare}[1]{%
  \def\graphname{#1}%
  % \def\nlandmarksA{#2}%
  % \def\nlandmarksB{#3}%
  \subfloat[#1: validation]{
    \begin{tikzpicture}
      \begin{axis}[
        height=2in,width=2in,
        xtick = {2,4,...,10},
        minor x tick num = {1},
        xlabel = Embedding Dimension,
        ylabel = MSE,
        legend pos = north east,
        cycle list name = my cycle,
        ]
        
        \addplot+[hypy-color,mark min=above]%,mark options={solid,fill opacity=0}]
        table[x = dimension, y = validation_MSE]
        {../figdata/hypy_\graphname_L100_data.txt};
        
        \addlegendentry{$\ell = 100$}

        % \addplot+[hypy-color-L200,mark min=above]%,mark options={solid,fill opacity=0}]
        % table[x = dimension, y = validation_MSE]
        % {../figdata/hypy_\graphname_L200_data.txt};
        
        % \addlegendentry{l = 200}

        \addplot+[hypy-color-L400,mark min=above]%,mark options={solid,fill opacity=0}]
        table[x = dimension, y = validation_MSE]
        {../figdata/hypy_\graphname_L400_data.txt};
        
        \addlegendentry{$\ell = 400$}

        \addplot+[hypy-color-L800,mark min=above]%,mark options={solid,fill opacity=0}]
        table[x = dimension, y = validation_MSE]
        {../figdata/hypy_\graphname_L800_data.txt};
        
        \addlegendentry{$\ell = 800$}
        
        % \pgfplotsset{cycle list shift=-1}
        % \addplot+[hypy-colorB,mark min=below]
        % table[x = dimension, y = validation_MSE]
        % {../figdata/hypy_\graphname_L\nlandmarksB_data.txt};
        
        % \addlegendentry{Hypy, l = \nlandmarksB}
        
      \end{axis}
    \end{tikzpicture}
  }%
}

% Special Commands to Mark the Min or Max of a Plot
% http://tex.stackexchange.com/questions/46176/pgfplots-mark-max-min-value-of-a-function
\makeatletter
\pgfplotsset{
    compat=1.12,
    /tikz/max node/.style={
        anchor=south,
    },
    /tikz/min node/.style={
        anchor=north,
        name=minimum
    },
    mark min/.style={
        point meta rel=per plot,
        visualization depends on={x \as \xvalue},
        scatter/@pre marker code/.code={%
            \ifx\pgfplotspointmeta\pgfplots@metamin
                \def\markopts{}%
                \coordinate (minimum);
                %\node[#1]{$\ast$};%
                \node[#1]{\tiny  min};%
            \else
                % \def\markopts{mark=none}
                \def\markopts{}
            \fi
            \expandafter\scope\expandafter[\markopts,every node near coord/.style=green]
        },%
        scatter/@post marker code/.code={%
            \endscope
        },
        scatter,
    },
    mark min/.default={below},
    mark max/.style={
        point meta rel=per plot,
        visualization depends on={x \as \xvalue},
        scatter/@pre marker code/.code={%
        \ifx\pgfplotspointmeta\pgfplots@metamax
            \def\markopts{}%
               \coordinate (maximum);
                \node[#1] {(\pgfmathprintnumber[fixed]{\xvalue},\pgfmathprintnumber[fixed]{\pgfplotspointmeta})};%
        \else
            %\def\markopts{mark=none}
            \def\markopts{}
        \fi
            \expandafter\scope\expandafter[\markopts]
        },%
        scatter/@post marker code/.code={%
            \endscope
        },
        scatter
    },
    mark max/.default={above},
}
\makeatother


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

